Scaling of Entanglement-Assisted Communication in Amplified Fiber Links

Quantum information processing technology offers several communication strategies, which offer capacity advantages over classical technologies. However, advantages typically arise only in very particular communication scenarios which are of limited use in public networks. Most importantly, striking capacity advantages have so far been found only for cases where the system capacity is way below commercially interesting values. In this work we present a novel scenario where pre-shared entanglement offers arbitrarily high capacity advantages, and where at the same time data rates are compatible with future network demand. Our approach rests on the observation that the number of modes in multi-mode fiber can be increased solely by tuning of the refractive index, while maintaining the fiber diameter.

==> attic/v1_03_CEA_approximation.tex <==
\section{Formulating an approximation for $C_E$}


We aim to estimate $C_E$ with high accuracy, enabling us to analyze its asymptotic scale as the number $M$ of orthogonal channels subject to global power constraint (${\Sigma_{m=1}^M P_m \leq P}$) increases. The scaling of the overall system capacity with $M$ channels is, in this case described by the quantities $C_X(M,P,\tau,\nu)$. For the system using \ac{SSR} and \ac{JDR} (${X\in \{S,J\}}$) the capacity scaling has been stated in \cite{ntzel2022operating}, where
\begin{equation}
    \lim_{M\to\infty} C_H(M,P,\tau)= \tfrac{P}{M} \cdot \tau \log(\tfrac{1+\nu}{\nu}).
\end{equation}
%%% COMMENT ON THE NOISE CALCULATION ONCE THE Noise is understood
This value sets the true benchmark for entanglement-assisted communication to provide an advantage in terms of the data transmission capacity. The question is thus for which values of ($M,P,\tau$) the entanglement-assisted capacity can outperform the non-assisted capacities by a given factor. As one can see from Equation \eqref{eq:C_E}, it can be helpful to understand the individual scaling of the involved four terms. In this analysis, we study the terms:
\begin{align}
    &{M\big(g(\tfrac{P}{M}) -g(d_{0}(\tau,\tfrac{P}{M},\nu))\big)}\text{ and }\\
    &{M\big(g(\tau \tfrac{P}{M} + \nu) -g\big(d_{1}(\tau,\tfrac{P}{M},\nu))\big)},
\end{align}
separately.

Our approximation rests on the following observations: For every $\tau \in [0, 1] $ and $\nu \geq 0$ it holds $d(\tau, 0, \nu) = 0$, which would further imply $d_{1}(\tau,0,\nu)=0$.

Our second observation is that the derivative of $d_{1}(\tau,n,\nu)$ at $n = 0$ satisfies:
\begin{equation}
    \partial_n d_{1}(\tau, n,\nu)|_{n=0} = \tfrac{(1+\nu - \tau)}{(1+\nu)}.
\end{equation}

Since $\lim_{\epsilon \to 0 } g(\nu + \epsilon) = g(\nu)$
